Quiver: Supporting GPUs for Low-Latency, High-Throughput GNN Serving with Workload Awareness

Systems for serving inference requests on graph neural networks (GNN) must combine low latency with high throughout, but they face irregular computation due to skew in the number of sampled graph nodes and aggregated GNN features. This makes it challenging to exploit GPUs effectively: using GPUs to sample only a few graph nodes yields lower performance than CPU-based sampling; and aggregating many features exhibits high data movement costs between GPUs and CPUs. Therefore, current GNN serving systems use CPUs for graph sampling and feature aggregation, limiting throughput. We describe Quiver, a distributed GPU-based GNN serving system with low-latency and high-throughput. Quiver's key idea is to exploit workload metrics for predicting the irregular computation of GNN requests, and governing the use of GPUs for graph sampling and feature aggregation: (1) for graph sampling, Quiver calculates the probabilistic sampled graph size, a metric that predicts the degree of parallelism in graph sampling. Quiver uses this metric to assign sampling tasks to GPUs only when the performance gains surpass CPU-based sampling; and (2) for feature aggregation, Quiver relies on the feature access probability to decide which features to partition and replicate across a distributed GPU NUMA topology. We show that Quiver achieves up to 35 times lower latency with an 8 times higher throughput compared to state-of-the-art GNN approaches (DGL and PyG).

==> sections/api.tex <==
% Section 5

\section{Unified Tensors}

% This is however challenging because these GL libraries have their own tensor and task implementations.  As a result, emerging distributed GL systems, \eg P3~\cite{p3} and AliGraph~\cite{aligraph} have to require users to rewrite GL applications.  Alternatively, the users can use RPC libraries such as gRPC and PyTorch RPC to integrate components from different libraries (\eg using the GPU sampler from DGL in AliGraph), but suffering from large performance overheads.

% A design goal of \sys is to support the large number of GL applications
% that have been implemented by PyG and DGL.

To reduce performance overheads when supporting GL jobs that use the PyG and DGL frontends, \sys uses efficient \emph{unified tensors}. Unified tensors are based on the following observation: although GL tasks are implemented using different APIs in PyG and DGL, their underlying data structures are tensors that store the graph topology, features and GNN models. Therefore we can design a tensor as a replacement for the different tensor types (\eg \code{DGLGraph} in DGL~\cite{dgl} and \code{SparseTensor} in PyG~\cite{pyg}). We can thus allow PyG and DGL tasks to access data transparently within \sys tensors and, under the hood, \sys then re-directs data accesses to different devices at runtime.

% Next, we describe the implementation of unified tensors, introduce the APIs of \sys and describe how to use \sys in existing GL jobs.

%There are many GL models from various libraries. The design goal of \sys's API is to allow users to integrate existing GL models with minimal efforts. To achieve this, \sys supports unified tensors which are compatible with most popular GL libraries, and these abstractions enable the optimisations by \sys which have been mentioned previously. We also provide API examples to explain how to modify a few lines of code from another GL library so that \sys could boost its performance.

% \begin{figure}[tbp]
%   \includegraphics[width=\linewidth]{figures/support.pdf}
%   \caption{Data access with unified tensors}\label{fig:support}
% \end{figure}

% Supporting heterogeneous GL models
% Hybrid task supported
% Data access issues
% Providing unified tensor

%\subsection{Supporting heterogeneous GL models}
%
%Existing GL libraries usually provide graph data and GL computation APIs to support heterogeneous GL models. To represent the graph topology, they provide high-level graph APIs (\eg \texttt{DGLGraph} in DGL~\cite{dgl} and \texttt{SparseTensor} in PyG~\cite{pyg}) so that graph construction and transformations are available to users. Graph features are represented as tensors, so that users can access the features by tensor operations. To support represent GL computations, they mainly provide samplers (\eg random walk sampler nad k-hop neighbour sampler) and graph neural networks (\eg graph convolution or graph attention modules) so that users can build an end-to-end GL pipeline by combining these modules.
%
%It is challenging to integrate both graph data and GL computation from various GL libraries, because there are no standard graph data formats and computation specifications. However, \sys provides a general graph data representation at lower level, so that every graph data structure will built on top of \sys's data layer, and every computation module could access graph data transparently. Next, we will explain how our general graph data representation works.

% In \F\ref{fig:support}, to integrate our system optimisations with exisiting GL libraries, \sys introduces \emph{unified tensor} and \emph{unified task} abstractions. With unified tensors, both graph structure and graph features could be unified into the same graph data representation, which will be managed by \sys's data management module. Unified tasks help \sys integrate exisiting GL samplers and models with our task dispatchers. Since feature aggregation is to access graph data and it is controlled by \sys's unified tensor, all three types of GL tasks are handled by \sys's task dispatching pipeline.

% \subsection{Unified tensor implementation}

%We first discuss how to represent all GL data structures as tensors. Graph data includes graph structure and graph features. Graph features are dense tensors that have been well supported by ML frameworks. Graph structures are sparse, but they are usually represented as dense tensors as well (\eg \textit{CSR} or \textit{COO} format). 

\sys provides a distributed and transparent unified tensor abstraction for data spread across local and remote device memory, thus allowing GL tasks to run with \sys without modification. As shown in \F\ref{fig:support}, the GL tasks always operate on a large local tensor object but \sys tensors implement three types of efficient data access:

\mypar{Local data access} GL tasks often access tensors that are larger than the local GPU memory. For example, a GPU-based graph sampling task may need to sample nodes on a large graph. To support this, \sys support a ``local'' data access strategy (\myc{1} in \F\ref{fig:support}) to data stored in local GPU memory, on-host CPU, disks and remote servers.

To support a data lookup on this large tensor, \sys uses a tensor index, which divides the tensor into index ranges. Each range is associated with the memory space of a specific device. If some tensor items fall within the range of a device, corresponding memory access are generated. To improve the performance of cross-device data accesses, \sys tensors exploit low-level hardware features of GPUs, \eg CUDA's zero-copy access technology. For example, PCIe requests are issued automatically when a worker accesses the elements on CPU memory; GPU data is accessed with a GPU memory address. For disk data access, the data range is memory-mapped into paged virtual address space, and the accessed data page is swapped in on-demand.

\mypar{Multi-process data access} GL jobs can also launch multiple Python processes, and these processes need to share data using tensors. For example, many jobs rely on data-parallel training in which each training process is assigned to one GPU. These training processes must aggregate features, and some features can be owned by other processes. \sys tensors thus must provide multi-process support (\myc{2} in \F\ref{fig:support}).

Multi-process data access is, however, challenging due to the overheads from excessive data serialisation/deserialisation and slow OS data movement calls. \sys places data into OS shared memory so that  processes can access it. To make the data accessible from GPUs, \sys page-locks the data so that it becomes accessible by the CUDA kernels of any GPU in the server. To share GPU data, \sys handles two cases: (1)~when two GPUs can directly access each other (\eg under the same PCIe switch or connected via NVLink), the tensor address is shared with the CUDA IPC~\cite{cudaipc} mechanism, and zero-copy access is supported; and (2)~otherwise, \sys sends GPU data requests from one worker to a remote one, and lets the remote worker collect requested GPU data and responses when they are ready.

\mypar{Inter-server data access} When GL jobs use multiple servers for training large GNN models, \sys tensors must support efficient data access to remote servers (\myc{3} in \F\ref{fig:support}). For this, tensors can be expanded via heterogeneous networks (\ie InfiniBand and Ethernet). \sys uses the NCCL~\cite{nccl} library to achieve this because NCCL automatically detects server configurations and chooses optimal communication topologies.

A challenge is that GL jobs may have irregular data access patterns, \ie the network messages are not symmetric and fixed-length. This makes it difficult to use NCCL's collective communication primitives because they assume symmetric communication and equal-sized messages. To address this, \sys relies on an inter-server network stack for unified tensors, which adopts low-level NCCL primitive, \ie \code{send}/\code{recv}. If one process must access the graph data from another server, it sends the indices of the requested elements. On receiving the request, the responder asynchronously finishes the inter-server data access. \sys schedules all requests and responses to saturating the cluster bandwidth.

% \sys could also schedule multiple peer-to-peer communication groups at the same time to fully utilise all available network bandwidth of the whole cluster.

% \subsection{Unified task abstraction}

% Existing GL libraries often support both CPU and GPU task implementations for GL tasks. Since \sys's hybrid parallelism will dispatch CPU and GPU tasks, it is necessary to support \emph{unified task} abstraction in \sys. This is challenging because each GL library has its own input and output specification for GL computation. \sys does not require users to manually transform any GL task implementation from another GL library to meet \sys's specifications. Users only need to run an example program from a GL library as usual, but this time with \sys's classes such as samplers and features. These classes are actually task executors which follow the original computation logic, but what they execute are the unified tasks, with an additional argument indicating which processor.

% When users create a task executor in a worker, the constructor arguments might not be sufficient for \sys's hybrid parallelism (\eg users may provide graph structure which could only be accessed by CPUs), so the executor will perform necessary data transformations and allocations based on the requirements of both CPU and GPU tasks. The executor will also try to connect to \sys's local dispatcher. During the training time, when the executor receives a batch of input data, it will follow the dispatching results from local dispatcher and split the batch. Similar to class construction, before launching a CPU or GPU task, the executor will check the input micro-batch and sometimes transform it.

% \subsection{Minimal code change to adopt \sys}

% \sys's unified tensors allow existing PyG and DGL applications to easily adopt \sys as the underlying
% distributed execution engine. This makes \sys quickly become the officially recommended distributed library for PyG, and it has been endorsed by the DGL community. 
% \notelx{Does this violate double blind reviewing?}
% To enable \sys in a PyG application, for example, the PyG users only need to write a few lines of new code (usually 3 - 5 LoC):
% (1)~They replace PyG's graph sampler with \sys's graph sampler (which replaces PyG default tensors with \sys tensors), and (2)~They replace PyG's feature objects.
% In this \sys program, PyG's GNN models, sampling functions and feature processing functions can be used without modification.
% % single-GPU python script

%\usemintedstyle{vs}
%\begin{listing}[t!]
%
%\begin{minted}[mathescape, linenos, numbersep=5pt, frame=lines, framesep=2mm, fontsize=\scriptsize, baselinestretch=.7]{python}
%
%import quiver
%
%## Step 1: Replace PyG graph sampler
%# train_loader = NeighborSampler(data.edge_index, ...)
%train_loader = quiver.NeighborSampler(data.edge_index, ...)
%...
%
%## Step 2: Replace PyG feature collectors
%# feature = data.x.to(device)
%quiver_feature = quiver.Feature([device]).from_cpu_tensor(data.x)
%...
%  
%## Step 3: Train PyG models with Quark
%for batch_size, n_id, adjs in train_loader:
%  batch_feature = quiver_feature[n_id]  # Access Quark feature
%  out = SAGE(batch_feature, adjs)  # Use PyG original SAGE model
%...
%\end{minted}
%\caption{\sys's example program}\label{lst:example}
%\end{listing}


==> sections/autobatch.tex <==
\section{Autobatching}

% Why not fixed batch size?
% 1. model hyperparameters - different number of sampling
% 2. Feature dimensions
% 3. Dynamic requests from clients
% -- Latency aware - Fixed batch size causes large latency

% Why CPU and GPU hybrid sampler? CPU vs GPU sampling
% CPU small batch
% GPU large batch

% Runtime determination of batch size, CPU or GPU
% Runtime monitoring of requests
% - average latency
% - throughput
% - queuing size
% Description of the strategies (structure figure)
% - How to determine the batch size?
% - How to determine which queue to input?

==> sections/data.tex <==
% Section 3

\section{GPU-NUMA-Centric Feature Store}

We want to avoid communication bottlenecks when processing GNN feature requests. For this, \sys uses a \emph{GPU-NUMA-centric feature store} that partitions and replicates features on the GPUs and CPUs and supports one-sided reads over NVLink, PCIe and InifiniBand. 

Figure~\ref{fig:feature-store} gives a design overview of the \sys feature store. The feature store contains a feature placement manager~(shown by \myc{1}). The placement manager estimates the \emph{access probability} of features and takes the device topology of GPU-NUMA servers into account.  It then partitions the features and places feature partitions into the CPU memory of servers, ensuring balanced access probabilities across servers. The feature store also replicates hot features based on their access probabilities in the CPU and GPU memory. The placement of features is recorded in a \emph{feature lookup table}, which is replicated on each server.

When \sys processes requests, its GPU kernel for feature collection retrieves remote features through the feature store (shown by \myc{2}). The kernel uses the feature IDs (usually the graph node IDs) for lookups in the feature table. The table returns the physical location of features and the closest location when multiple replicas exist. Based on the location,
the kernel use \emph{one-sided GPU/CPU/RDMA reads} to collect the features from local GPUs (NVLink), local GPUs (PCIe) and remote CPU (InfiniBand), respectively. Since using InfiniBand and PCIe both heavily involves look-aside buffer~(TLB) lookups, the feature store \emph{reorders features} before reading them remotely, optimising TLB hit ratios. 

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{arxiv/figures/quark-feature-store.pdf}
  \caption{Design of the feature store}\label{fig:feature-store} 
\end{figure}

\subsection{Feature placement manager}

\sys computes feature access frequencies to estimate which features are more likely to be collected when serving GNNs. It leverages the access frequencies to optimise feature placement on the GPU-NUMA servers.

\subsubsection{GNN feature access probability}

Estimating feature access probabilities for GNN serving involves several challenges: (i)~different from existing approaches (\eg PaGraph~\cite{pagraph}, GNNLab~\cite{gnnlab} and BGL~\cite{bgl}) which take training datasets to estimate the probabilities (or frequencies), serving systems do not have serving datasets when estimating the probabilities, and they suffer from performance degradation when performing online estimation; and (ii)~serving systems can take different parameters for configuring the graph sampling function (\eg different numbers of sampling layers or different probabilities for choosing a neighbour). This makes the probability estimation different from training scenarios in which users reuse the confi guration of the graph sampling function for GNN model training~\cite{gnnlab, pagraph, bgl}.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{arxiv/figures/quark-access-probability-intuition.pdf}
  \caption{Intuition behind the access probability calculation}\label{fig:probability} 
\end{figure}

To overcome these challenges, we design an \emph{analytical} access probability estimation method. This method does not rely on serving or training datasets, and it can be generalised to different multi-layer sampling functions commonly used in production GNN systems.

% \[
%     P(n, j)=
% \begin{dcases} 
%     P(n,j-1) + \left [ 1-P(n, j-1) \right ] \times \\
%     \left [1 - \prod_{s\in\mathcal{N}_n }(1-P(s,j-1)\times R(s, n) ) \right ],& \text{if } j>1\\
%     \frac{1}{|V|} ,  & \text{if } j=1
% \end{dcases}
% \]

We first describe the intuition in Figure~\ref{fig:probability}. Consider that we want to compute the probability that the graph node~$A$ is sampled as a neighbour within 2~layers, denoted as $P(A,2)$. This probability is the sum of (i)~the probability that it is sampled as a layer-1 neighbour: $P(A,1)$ (shown as \myc{1}), and (ii)~the probability that it is sampled as a layer-2 neighbour and not a layer-1 neighbour (shown as \myc{2}). More specifically, $1 - P(A,1)$ is the probability that node~$A$ has not been included as a layer-1 neighbour. $P(B,1) \times 0.5$ (shown as \myc{3}) is the probability that node~$A$ is sampled from node~$B$ with a probability of $0.5$ (since node~$B$ has 2~neighbours in total), and node~$B$ is sampled as a layer-1 neighbour.

We generalise the above intuition to derive the probability for a graph node (or edge) to be sampled within a given number of layers as:
\[
    P(n, j)=
\begin{dcases} 
    P(n,j-1) + \left [ 1-P(n, j-1) \right ] \times \\
    \left [1 - \prod_{s\in\mathcal{N}_n }(1-P(s,j-1)\times R(s, n) ) \right ],& \text{if } j>1\\
    \frac{1}{|V|} ,  & \text{if } j=1
\end{dcases}
\]
where $P(n,j)$ donates the probability that the graph node (or edge) $n$ is sampled as a neighbour within $j$ layers. The first term is the probability that $n$ is sampled as a layer-$j-1$ neighbour. The second term is the probability that $n$ is sampled as a layer-$j$ neighbour but not as a layer-$j-1$ neighbour, which is the product of the probability that $n$ is not sampled at layer ($1 - P(n,j-1)$) and that $n$ is sampled from any of its neighbours $\mathcal{N}_n$. For $j > 1$, the last probability is calculated by the probability of each $n$'s neighbour $s$ being sampled as a layer-$j-1$ neighbour ($P(s,j-1)$) and the probability that $n$ is sampled from $s$ ($R(s,n)$). For $j=1$, it is the uniform probability over the nodes ($1/|V|$).

\mypar{Practical considerations} To make access probability useful in practice, we make the following improvements to the above algorithm: (i)~the algorithm can take different parameters in configuring how a neighbour is chosen (\eg sampling the neighbour based on edge weight); and (ii)~the algorithm can use GPUs to parallelise probability calculation, making it possible to analyse large graphs in production environments. 

% \sys takes the sampling function implemented in PyG and DGL to e

% \mypar{Access probability estimator}
% \begin{itemize}
% \item {How to estimate access frequency using a white-box approach?}
% \item {How the estimator executes in parallel to reduce overhead?}
% \end{itemize}

% Knowing which features will be frequently accessed is the key to both load-balancing and improving access locality. Existing approaches estimate access frequencies only by the graph structure, or they need expensive pre-sampling. However, since the types of samplers in real-world GNN inference are limited, \sys applies white-box frequency estimators to solve the problem, with the sampler type and hyper-parameters as inputs. It takes both the graph structure and the sampler into account, without the need to actually run the samplers. \sys requires the sampler's type to choose the right estimator, and hyper-parameters as the arguments of the estimation function. \sys implements a few estimators for difference sampler types, covering most of the GNN models.

% Once an estimator is chosen, it will read the neighbours of each node, iteratively update the current access frequencies of all nodes by sampler hyper-parameters and finally write the result to the frequency table. We observe that most of the GNN samplers work in an iterative way, so our frequency estimation is also done similarly: first we initialise an access frequency table with equal values, then we analyse what updates need to be applied to each node's latest frequency value according to the sampling hyper-parameters in each iteration. For example, for multi-layer neighbour sampling estimators, if the neighbours of a node are likely to be accessed at the previous layer, this node's frequency will be updated to a higher value at this layer. The exact value is calculated with the hyper-parameters, \ie how many neighbours of each node will be sampled at this layer.

% The frequency computation of \sys's estimators are highly parallelizable because the update of each node frequency value is independent of each other in the same iteration, though there might be dependencies between iterations. Based on that computation logic, \sys implements all types of estimators as GPU kernels, in a node-parallel or edge-parallel way. They read the graph structure in CPU memory to obtain neighbourhood information while updating the frequency table in GPU memory. GPUs usually have a number of GiBs of memory, and the space complexity for GPUs is linear to the number of nodes in the graph, so it could handle graphs with billions of nodes. The overhead of frequency estimation is just a few seconds after the graph structure is loaded into CPU memory, thanks to the massive parallelism of the computation on GPUs.

\subsubsection{Optimised feature placement}

% The feature placement in \sys aims to: (i) balance the graph data access across servers so there is no straggler in the feature collection stage, which will reduce tail latency; (ii) improve feature locality to reduce the I/O latency incurred by remote feature access. To achieve these goals, \sys first estimates the access frequencies of all the nodes in the graph using a white-box approach. It then uses the frequencies to evenly partition the features across servers. Finally, with the extra memory of CPUs and GPUs, \sys decides which features to place on them to further improve feature access locality.

% Before the inference service is deployed, \sys loads the graph structure into CPU memory. \sys uses the graph and the sampler type and hyper-parameters of the GNN model to compute the access frequency table of all the nodes. The estimation algorithm is massively parallel, and it could be executed on GPUs. This table is then accessed by an intra-server partitioning algorithm to decide how to partition all features across servers. After partitioning, each server will know which features to store in its CPU memory, and on each server, there will still be some extra CPU memory and GPU memory left. \sys decides which features to replicate in these memory, also with the help of the access frequency table. The extra CPU memory is to replicate remote features, while the extra GPU memory is to replicate local features which placed on local CPU memory. After feature partitioning and replication is decided, each server will load the corresponding features from feature storage to serve feature collection during inference.

When placing features on GPU-NUMA servers, we want to load balance and ensure data locality, both of which are key requirements for a GNN serving system. Our placement follows the following steps:

\mypar{(1)~Partitioning and replicating features on distributed servers} \sys partitions features that can not be fitted in a server. Conventional partitioning approaches either randomly assign features to servers or use graph partitioning algorithms~\cite{karypis1998fast} that compute a min-cut for the graphs. In our production environments, we observe that the former leads to poor data locality and the latter is expensive to run, given the graph sizes.

\sys adopts a practical approach optimised for GPU-NUMA servers. It loads balances across the servers while optimising data locality by allowing \sys GPUs to maintain hot features in local host memory. We over-subscribe the servers and use a range-partitioning method to split the features. Since servers are over-subscribed, each server has free memory after partitioning. We sort the features based on their access probabilities. For each server, we replicate hot features that have not yet been assigned to this server until all its memory has been exhausted.

\mypar{(2)~Replicating features in GPU memory} \sys further replicates hot features in GPU memory (HBM), which improves GPU data locality. For GPUs in a NUMA socket, we take a different approach for replicating features: (i)~if NVLInk is available for the GPUs in this socket, reading features from peer GPUs is extremely efficient. We thus sort features based on access probabilities and evenly assign hot features to these GPUs until all their memory have been used; and (ii)~if NVLink is unavailable for the GPUs in this socket, reading features over PCIe can become a bottleneck. We thus replicate hot features in every GPU until the memory is full.

\subsection{One-sided reads of features}

\sys supports different one-sided reads of features, which efficiently utilise the multiple DMA paths available in GPU-NUMA servers. 

\subsubsection{Feature lookup table}

\sys supports one-sided reads used by feature collection kernels through a feature lookup table. The kernel uses a \emph{mask tensor} to decide if  collected features reside locally. If they are not local, it queries the feature lookup table. The table translates the feature IDs to the physical memory addresses on devices without involving CPUs. With the physical addresses, the GPU kernel can use one-sided read techniques that minimise memory copies to access the features on remote devices directly.

\mypar{Computing memory address} When \sys is deployed, each server constructs a feature lookup table, which maps each feature ID to (i)~the device storing the feature; and (ii)~the address of the feature on that device. Both are represented as integers in each row of the table.

\mypar{Memory and lookup costs} The number of rows in the lookup table is equal to the number of graph nodes. Therefore, the space complexity of the table is linear to the number of nodes, which is less than the space for the whole graph structure. The row number of the device and pointer of one node is the same as the feature ID, so lookups are completed in constant time. A batch of feature address lookups can be executed in parallel by the CPUs.

\subsubsection{Making one-sided reads efficient}

Although one-sided reads are available for GPUs, using them efficiently when GNN features are large remains challenging. Next, we discuss how to realise sided read over NVLink, PCIe and InfiniBand, and how to make them efficient by taking GNN computation and communication characteristics into account. 

% \mypar{One-sided remote feature read}
\mypar{One-sided GPU reads with NVLink} A GPU directly reads the memory of an NVLink GPU from a CUDA kernel, and the reads is finished with low latency and high throughput.

\mypar{One-sided local CPU reads with PCIe} The CPU features are registered as pinned memory using \texttt{cudaHostRegister}, allowing the CUDA kernels on local GPUs could to access all of them directly. Before reading a batch of features from registered host memory, the requested features are sorted according to their addresses, achieving better locality during address translation of GPUs.

\mypar{One-sided remote CPU reads with InfiniBand} The CPU features are also registered as a memory region using \texttt{ibv\_reg\_mr} for InfiniBand. \texttt{ibv\_post\_send} is called to perform a one-sided read. This reduces the time needed for memory copies and CPU intervention because, unlike RPC-based methods, it does not require the remote CPUs to gather the requested features on that machine and send them. \sys allocates multiple queue pairs to parallelise RDMA reads, improving throughput. Instead of setting the signal field and polling the completion queue for each read, \sys performs it once for each batch to reduce latency. To improve the TLB hit rate of the NIC, all reads are also sorted by remote feature addresses.

% \section{Optimising Data Accesses}
% \label{sec:data_accesses}

% %\subsection{Design overview}

% % We describe  propose \sys, a novel workload-aware distributed GL system, in which the allocation of GL data to CPU and GPU devices is optimised according to runtime analysis of GL workloads.

% The design of \sys{}'s data access approach aims to achieve several goals: (i)~reducing the time for remote data access across the whole training pipeline (\ie including remote sampling and feature aggregation); (ii)~balancing the data access costs of all data-parallel workers; and (iii)~minimising the overheads form pre-processing and allocating data.

% % (i)~The runtime analysis not only consider graph topology but also training datasets, user-defined graph sampling/traversal functions,
% % device topology and CPU/GPU configurations; 
% % (ii)~The algorithms need to be general so that
% % they can be applied to most GL applications, and help these applications
% % achieve load balancing and low communication cost for CPU/GPU devices; 
% % (iii)~The runtime analysis and data allocation need to minimise performance overhead,
% % and avoid manual data pre-processing.

% %\sys adpopts \emph{workload-aware} data management when deciding on how to partition and replicate graph data across GPUs and GPUs. To achieve this goal, several requirements have to be met: (i)~minimise the data access latency of sampling and feature aggregation; (ii)~avoid stragglers caused by imbalanced data placement; and (iii)~reduce the cost of integrating the data management in the training pipeline. \sys achieves them by efficiently analysing user-defined workloads and automatically finding out the optimal data management decisions.

% \begin{figure}[t]
%     \includegraphics[width=\linewidth]{figures/data.pdf}
%     \caption{Overview of data allocation in \sys}\label{fig:data}
% \end{figure}

% \F\ref{fig:data} shows how \sys performs data allocation. The intuition is that \sys obtains the data access pattern by analysing the workload. It uses a probability estimation algorithm, which takes the training dataset, the sampling functions and the graph topology~\myc{1} as input and estimates the data access probability associated with specific graph vertexes or edges~\myc{2}. The graph data, with probabilities derived from the last step, is passed to a data partitioning and replication algorithm~\myc{3}. It considers the device topology and CPU/GPU configuration, computes a balanced cut of graph vertices, edges and features, and assigns the partitions to CPU and GPU devices. Most accessed graph data is replicated, thus minimising cross-device communication costs. Since the data allocation is integrated into the execution of the training program, it avoids extra data pre-processing steps.

% %There are three steps: (i)~probability induction, (ii)~graph data partitioning and (iii)~replication. Given the training dataset and the sampling function, \sys will traverse the graph and analyse data access probabilities (see \myc{1}), then vertex (edge) access probabilities will be associated with the graph. \sys utilises GPUs to accelerate the probability calculation in parallel. The second step is to partition the data across devices (see \myc{2}). Based on data access probabilities, the partitioning decision will be balanced and incur minimal data access latency. Finally, if there is still available memory on some devices, \sys will replicate graph data on them (see \myc{3}). The replication step futher improves graph data access locality with device topology and memory capacity information. Step \myc{2} and \myc{3} are actually executed at both inter-server and intra-server level in a distributed manner. All data management procedures are integrated into the training pipeline with low overheads.

% \subsection{Data access probabilities}

% % 4 - 5 sentences to discuss the motivation for probability
% % 1. Consider both graph topology and GL application information
% % 2. General enough
% % 3. Low data pre-processing cost

% % First key point: Define probability (defintion)

% % Second key point: Example

% % Parallel algorithm declaration

% %The core idea of \sys's \emph{workload-aware} data management is to calculate the access probabilities of graph data. While existing graph data management solutions (\eg DGL~\cite{dgl} and Aligraph~\cite{aligraph}) only take the graph topology into consideration when they partition and replicate graph data, we observe that the training dataset and the sampling algorithm also play an important role in deciding the access probabilities of graph data.

% The data access patterns of GL tasks (\ie graph sampling and feature aggregation) depend on the models and datasets, \eg the number of graph vertexes to sample, the depth of sampling neighbours and the labelled vertices in the training datasets. To estimate data accesses, we require an algorithm that jointly analyses graph topology, models and datasets, yet incurs low time and space complexity. To achieve this, we propose:

% % This is because sampling functions may traverse the graph beginning from the labelled vertices in the training dataset, and they adopt diverse traversal approaches and hyper-parameters. Secondly, the solution using graph data probabilities has to be general enough, so that most GL applications can benefit from \sys's graph data management. Finally, the overheads of calculating the data access probabilities should be low, and it should be easily integrated into the training pipeline, so users will not be blocked by this pre-processing step.

% \mypar{Probability calculation} Data access probabilities are the probabilities of how frequently a vertex/edge is accessed during GL. Given a graph $G(V,E)$, a sampling function~$S$ (\eg how to sample from one seed vertex), a training dataset~$T$ (\eg labelled vertices), the probability for accessing a vertex~$v_0$ (or an edge~$e_0$) in training can be represented as:

% \noteprp{can you simplify the notation? mathcal should only be used if you run out of regular letters; $N_{access}$ is not defined; why does it need to have the subscript `access`? what is the semantics of the semicolon in (1)?}

% %\begin{equation}\label{eq:prob}
% %    \mathtt{PROB}_{v_0}(G, D, S) = \frac{\mathtt{access\_count}_{v_0}(G, D, S)}{\sum_{v \in V}{\mathtt{access\_count}_{v}(G, D, S)}}
% %\end{equation}

% \begin{equation}\label{eq:prob}
%     \mathcal P(v_0; G, T, S) = {\mathcal N_{access}(v_0; G, T, S) \over \sum_{v \in V} \mathcal N_{access}(v; G, T, S)}
% \end{equation}

% \noindent
% The probability is normalised by dividing the number of access by the total number of accessing over all vertices~$V$.

% It is possible to compute such probabilities for most GL jobs in production environments analytically, as explained below. Such jobs handle large datasets and models, and thus often use sampling-based GNN models---full-batch alternatives~\cite{gcn} are limited by GPU memory and thus cannot support large production datasets. Sampling functions result in different patterns traversing the graph, and these patterns can be quantified by associating a number with each vertex/edge that indicates how often it is traversed by a specific sampling algorithm. Although sampling functions are stochastic by nature, they decide on a probability distribution for all vertices and edges in the graph.

% \begin{algorithm}[t]\footnotesize
%     \DontPrintSemicolon
%     \KwIn{Graph $G(V,E)$; Training dataset vertices $T$; Sampled probability distribution from a vertex $S$; Number of sampling iterations $I$}
%     \KwOut{Vertex access probability $\mathcal P$}
%     $\mathcal P \leftarrow 0$\\
%     \For{$t \in T$}{
%         $\mathcal P_t \leftarrow {1 \over len(T)}$
%     }
%     \For{$i=1\;to\;I$}{
%         $\overline{\mathcal P} \leftarrow 0$\\
%         \For{$v \in V$}{
%             $\overline{\mathcal P} \leftarrow \mathcal P + S(v)$
%             % $weight \leftarrow vertex\_weight(S,v)$\\
%             % $sampled\_vertices \leftarrow sample\_all(S,v)$\\
%             % \For{$sv \in sampled\_vertices$}{
%             %     $p \leftarrow sample\_prob(S,v,sv)$\\
%             %     $\mathcal P_{sv} \leftarrow \mathcal P_{sv} + p * weight$
%             % }
%         }
%         $\mathcal P \leftarrow \overline{\mathcal P}$
%     }
%     \Return{$\mathcal P$}
%     \caption{\label{alg:prob}Probability calculation}
% \end{algorithm}

% \mypar{Parallel algorithm} An advantage of our approach for data access probabilities is that their calculation can be accelerated by using multiple GPUs. \A\ref{alg:prob} shows the probability calculation algorithm, which calculates the probability for graph vertexes.\footnote{The calculation for edges follows the same approach.} The algorithm first initialises the probabilities according to the dataset~(lines~2--3). For example, when using neighbour sampling, the probabilities of all labelled vertices are set to $1$ because all sampled subgraphs start from them. With these initialised probabilities, for each vertex, assigned weights indicate the probability of becoming the seed of the sampling function~(lines 4--5). It then samples all possible vertices from that vertex to obtain all reachable targets~(line~6). Next, it analyses the relative sampled probabilities of these vertices based on the sampling function and the seed vertex~(line~8). Finally, it updates the probabilities with both the weight and the relative probabilities~(line~9). Note that these three loops can be parallelised on GPUs by sharding along the dataset/vertex/edge dimensions.

% % \subsection{Probability-guided data allocation}

% % First 4 - 5 sentences to motivate the readers
% %1. Achieving load balancing on hybrid CPU and GPU devices
% %2. Achieving minimal communication cost, replication (consider device topology).
% %3. Low pre-processing cost

% % Optimising load balancing in the format of probability (definition)

% % Optimising communication cost ..... (definition)

% % Parallel algorithm declaration

% % \subsection{Data access probabilities}

% %  If static data management (\ie only graph structure is analysed) is applied to our GL pipeline, without looking at the training dataset and the sampling function, the data locality will be much worse and the performance will drop because of the cost of data transfer between local and remote devices.

% \subsection{Probability-guided data allocation}

% With the data access probabilities, \sys then partitions and replicates the data. Its goal is to minimise the cost of data access and to balance the data access across workers (\ie CPU and GPU devices). It also minimises the cost of making decisions about partitioning and replication.

% \begin{algorithm}[t]\footnotesize
%     \DontPrintSemicolon
%     \KwIn{\\
%       $N_g$: \#GPUs per server; \\
%       $N_s$: \#Servers; \\
%       $M_c$: CPU memory capacity; \\
%       $M_g$: GPU memory capacity; \\
%       $\mathcal T$: hardware topology; \\
%       $\mathcal P$: data access probabilities; \\
%       $C$: data chunk size} 
%     \KwOut{Data management decisions: GPU vertices $\mathbf{V}^g$, CPU vertices $\mathbf{V}^c$}
%     \SetKwFunction{Func}{partition\_and\_replicate}
%     \SetKwProg{myproc}{Function}{}{}
%     \myproc{\Func{$prob$, $ids$, $capacity$}}{
%     \If{$ids$}{
%         $prob \leftarrow prob[:,ids]$
%     }
%     $beg, end, rank, group \leftarrow 0, C, 0, dim(prob, 0)$\\
%     \While{$end \le dim(prob, 1)$}{
%         \For{$i=1\;to\;group$}{
%             $picker \leftarrow (rank+i)\mod group$\\
%             $order \leftarrow sort\_by\_prob(prob[picker], [beg:end])$\\
%             $\mathbf{V}_{picker} \leftarrow append(\mathbf{V}_{picker}, order[-\frac{C}{group}:])$
%         }
%         $beg, end, rank \leftarrow end, end+C, (rank+1)\mod group$
%     }
%     \If{$extra \leftarrow capacity - \frac{dim(prob,1)}{group},extra \ge 1$}{
%         \For{$i=1\;to\;group$}{
%             $order \leftarrow sort\_by\_prob(prob[i-1], [0: dim(prob,1)])$\\
%             $\mathbf{V}_{i-1} \leftarrow append(\mathbf{V}_{i-1}, order[-extra:])$
%         }
%     }
%     \If{$ids$}{
%         $\mathbf{V} \leftarrow ids[\mathbf{V}]$
%     }
%     \Return{$\mathbf{V}$}}
%     $M_s \leftarrow server\_capacity(T, N_g, M_c, M_g)$\\
%     \For{$i=1\;to\;N_s$}{
%         $\mathbf{S}_{i} \leftarrow \sum^{N_g}_{j=1}{\mathcal{P}_{ij}}$
%     }
%     $\mathbf{V}^s \leftarrow partition\_and\_replicate(\mathbf{S}, null, M_s)$\\
%     \For{$i=1\;to\;N_s$}{
%         $\mathbf{V}^s_i \leftarrow sort\_by\_prob(\mathcal{P}_i, \mathbf{V}^s_i)$\\
%         $\mathbf{V}^c_i \leftarrow \mathbf{V}^s_i[:M_c]$\\
%         $\mathbf{V}^g_i \leftarrow partition\_and\_replicate(\mathcal{P}_i, \mathbf{V}^s_i[M_c:], M_g)$\\
%     }
%     \Return{($\mathbf{V}^g, \mathbf{V}^c$)}
%     \caption{\label{alg:policy}Graph data partitioning and replication \noteprp{the notation is very lose here and needs cleaning up; ask me for details}}
% \end{algorithm}

% \mypar{Data access cost} Each worker has to access graph data, which is distributed across all devices. Data can be on a remote device or on local memory. We use data access time to measure, for a worker~$w$, the data transfer size~$S$ and the communication bandwidth~$B$, the average time spent on data access with all available devices~$D$:

% \noteprp{my use mathtt below?}

% \begin{equation}\label{eq:access}
%   % \mathtt{ACCESSTIME}(w) = \sum_{d \in D}{\frac{remote\_access\_size(D_w, d)}{bandwidth(D_w, d)}}
%   \mathcal{T}_{\mathtt{access}}(w) = \sum_{d \in D}{\frac{\mathtt{S}(D_w, d)}{\mathtt{B}(D_w, d)}}
% \end{equation}

% \mypar{Balancing data access} \sys balances graph data across workers to avoid stragglers that spend more time than others accessing distributed data. Formally, given the worker set~$W$, the balance metric to minimise can be represented as:

% \begin{equation}\label{eq:balance}
%     % \mathtt{BALANCE} = \frac{\max_{w \in W}{\mathtt{ACESSTIME}(w)}}{\min_{w \in W}{\mathtt{ACESSTIME}(w)}}
%     \mathcal{B} = \frac{\max{\{\mathcal{T}_{\mathtt{access}}(w) \mid w \in W\}}}{\min\{{\mathcal{T}_{\mathtt{access}}(w) \mid w \in W\}}}
% \end{equation}

% \mypar{Data allocation algorithm} Next, we discuss how to partition and replicate graph data based on the data access probabilities~$\mathcal{P}$. The input to the allocation algorithm are the hardware characteristics and the obtained probabilities, and it outputs the data allocation decisions, \ie which \noteprp{why is V bold here? use consistent notations, e.g. uppercase letters are sets and lower case letters are elements from sets} vertices~$\mathbf{V}^c, \mathbf{V}^g$ and edges to store on each device. The algorithm not only takes the estimated probabilities but also the hardware topology, \noteprp{why use 'bandwidth' spelled but it's B above?} $\mathcal T = \{\mathit{bandwidth}(d_1, d_2) \mid d_1,d_2 \in D\}$ and CPU/GPU memory capacities, $M_c, M_g$, into account.

% The algorithm first analyses the hardware characteristics and outputs server memory capacities~(line~18).
% %
% % \notezy{The key criteria are: if the inter-server connection is fast (\eg InfiniBand), the bottleneck is unlikely to be the inter-server communication, so the memory capacity of each server is given a low number to encourage intra-server data replication; if the intra-server connection is fast (\eg NVLink), \sys will aggressively parition intra-server data across GPUs (\ie larger server memory capacity), because inter-GPU communication has a much lower cost.}
% %
% The second step is that each server sums the probabilities of its workers~(lines~19--20). Inter-server partitioning and replication are subsequently performed (line~21). After that, on each server, CPU memory holds cold graph data; GPUs partition and replicate the rest (hot data) during the intra-server step~(lines~22--25). Finally, the CPU and GPU data placement decisions for all servers are returned~(line~26).

% Note that, the function $partition\_and\_replicate$ is used for both inter-server and inter-GPU partitioning and replication. The inputs are data access probabilities, vertex indices, and memory capacities of each device (server/GPU); the output is an array, with each element indicating which vertices to place on each device. The first part (lines~6--10) is about partitioning: in each iteration, starting from one device, each device selects a chunk of graph data with the highest access probability for itself. After every iteration, the same procedure begins with another device. Assigning resources round-robin based on probability order ensures that the partitioning is aware of the probabilities and also balanced. In the replication part~(lines~11--14), each device replicates the graph data with high access probabilities according to its own ordering, without the load-balancing constraint.

% \mypar{Data allocation example} As \F\ref{fig:data} shows, after sys has calculated all vertex probabilities, \ie each vertex is associated with a probability according to \A\ref{alg:prob}, it decides on how to partition and replicate the graph data~\myc{3}. After the execution of the \A\ref{alg:policy}, it partitions the graph into two disjoint sets of vertices, and the allocation algorithm ensures that the number of vertices (3:3) and the sum of vertex access probabilities ($1.4$:$1.7$) on CPU and GPU remains balanced. Furthermore, \sys replicates some data on both CPU and GPU memory---it decides to replicate two vertices (one with probability $0.8$ and the other $0.9$, which are frequently accessed but not stored locally) so that they can be accessed locally to reduce average data access latency.

% % Putting data near the worker

% % \subsection{Hardware-aware replication}

% % Meanwhile balancing all workers

% \mypar{Parallel computation} The intra-server partitioning and replication can be executed in a parallel fashion. Each server can decide on the data allocation for its own CPU and GPU memory without coordinating with other servers. Meanwhile, the inter-server allocation can be parallelised by sharding all vertices across servers. After the inter-server decisions are made for every vertex chunk in a distributed manner, the results are synchronised across servers. All workers now load their graph data partitions based on the output decisions from \A\ref{alg:policy} and begin the data-parallel training.

% % End


==> sections/eval/abla.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\hline
\textbf{Dataset} & \textbf{\sys} & \textbf{w/o InfiniBand/NVLink} \\
\hline
\textsf{mag240m} & 30.2\unit{ms} & 48.9\unit{ms} (w/o InfiniBand)  \\
\textsf{paper100m} & 27.4\unit{ms} & 41.2\unit{ms} (w/o NVLink) \\
\hline
\end{tabular}
\caption{Latency with different communication links \noteprp{I don't understand how this table works -- please fix}}
\label{tab:latency}
\end{table}



==> sections/multilink.tex <==
\section{MultiLink}

% We have cached hot data in multiple GPUs and servers.
% CNN workload is continuous in memory, GNN features are scattered over into multiple servers or GPUs.
% So GNN feature collection involves random memory accesses to different servers and GPUs

% Multi-GPU NVLINK and Multi-nodes RDMA are hard to utilise.
% Unified abstraction for feature tensors that supports nvlink and rdma loading transparently, localTensorPGAS, distTensorPGAS.
% - localTensorPGAS
% - distTensorPGAS



==> sections/task.tex <==
% Section 4

\section{Hybrid Task Scheduling}
\label{sec:scheduling}

Next, we introduce the task scheduling in \sys, which aims to achieve the following goals: (i)~schedule tasks that have both CPU and GPU implementations, deciding which implementation (or both) to use at runtime; (ii)~monitor task performance metrics and, based on monitored metrics, optimise the choice and assignment of task implementations at runtime; and (iii)~exhibit low runtime overhead, thus scaling to large clusters.

%To fully utilise heterogeneous processors, \sys takes an \emph{intra-batch hybrid parallelism} approach when assigning GL tasks (\ie sampling and feature aggregation) to processors. The goals of our hybrid parallelism design are: (i)~the training throughput each batch should be maximised; (ii)~the parallelism policy has to measure the task characteristics and predict the effects of any possible hybrid parallelism decisions; and (iii)~the policy should be executed efficiently. \sys manages to meet these requirements by modelling GL tasks effectively in our policy design, finding the optimal intra-batch hybrid parallelism decision and executing the policy in a decentralised approach.



\F\ref{fig:task} shows the design of \sys task scheduler. The \sys scheduler assumes GL jobs train GNN models using mini-batch SGD algorithms. The execution of a data batch \myc{1} is completed by the scheduler. A unique feature of the \sys scheduler is that it maintains a task implementation pool in which tasks (\ie sample and feature aggregation) have both CPU and GPU implementations \myc{2}. To utilise all available CPU and GPU devices, the scheduler partitions the data batch into micro-batches \myc{3}, and each micro-batch is assigned to a device. For the example of graph sampling, it can be completed by both CPUs and GPUs. The scheduler optimises the choice of micro-batch size and the assignment of micro-batches so that the data batch completion time is minimised (\ie maximising training throughput). The optimisation is guided by task metrics (\ie monitored task time, data locality information, estimated asynchronous execution time), and these metrics are computed at runtime, thus making the scheduler workload-aware \myc{4}.

%GL workloads usually take a distributed training pipeline with batch-based data parallelism: datasets are first divided into batches, and the training pipeline will execute one batch at a time to update the graph neural network iteratively. In \F\ref{fig:task}, a batch is further divided into micro-batches, and each micro-batch is assigned to a worker so that each work will train with a micro-batch in parallel. This batch-based scenario is adopted throughout the training pipeline (\ie all GL tasks follow this parallelism strategy). In a cluster with CPUs and GPUs, \sys fully utilises them by having micro-batch dispatchers that divide a batch to micro-batches (see \myc{1}). These dispatchers will dispatch micro-batch level computation tasks (sampling or feature aggregation) to both CPUs and GPUs, and they will let these tasks be executed on CPUs and GPUs simutaneously (see \myc{2}).
%
%The dispatchers will follow \sys's parallelism policy, which is adaptive to the workload by profiling and adjusting its dispatching methods dynamically. Therefore, runtime metrics have to be collected from heterogeneous processors (see \myc{3}). The dispatchers will receive these metrics which reflect workload characteristics and find the optimal dispatching strategy for incoming batches (see \myc{4}).

\subsection{Scheduler design}

% 4 - 5 sentences to motivate
% 1. Task interface to schedule tasks have two kernels
% 2. Low overhead

% Micro-batch idea

% Scheduler design architecture

%In GL, computation tasks sometimes have two kernel implementations (\ie one for CPU and the other GPU) when they could be executed on both CPUs and GPUs, however existing GL systems only choose one kernel to run throughout the training pipeline, which lead to processor under-utilisation. To utilise both CPUs and GPUs, \sys can integrate these hybrid GL tasks with our hybrid task scheduler. Meanwhile, \sys adopts intra-batch scheduling to balance the utilisation of hybrid processors.

There are two problems to be addressed in the design of the \sys scheduler: (i)~the task implementations often come from existing GL libraries, such as PyG and DGL, therefore we need a unified interface to import tasks from these libraries; and (ii)~\sys must have a general approach for allowing CPUs and GPUs to work jointly in completing GL tasks if tasks have both CPU and GPU implementations.

\mypar{Unified task scheduling interface}
%To support hybrid task scheduling, the first issue is that how \sys could make abstractions about hybrid GL tasks so that it can support them in general.
\sys wraps a GL task from PyG or DGL into its own schedulable task. Such a task has an attribute to denote whether it has a CPU or GPU kernel. If both CPU and GPU implementations are provided with the same functionality, \sys then schedules them together to fully utilise CPUs and GPUs. Since CPU and GPU implementations of the same task carry out the same computation, \sys only must perform the necessary data transformations so that the input data becomes accessible from both CPUs or GPUs. This approach is general in supporting all GL tasks because it does not require manual modification of existing task implementations while stilling enabling execution on heterogeneous devices.

\mypar{Partitioning data batch into micro-batches} The scheduler uses range-partitioning to divide a data batch into micro-batches. It places the micro-batches into the task queues of the selected CPU and GPU devices, giving a single micro-batch to each device. Micro-batch sizes determine how multiple devices collaborate to finish a task. For GL jobs, CPUs and GPUs may have similar throughput for some tasks; for deep learning jobs, GPUs may dominate the execution of compute tasks---GL computation is typically too irregular to utilise the full parallel computation potential of GPUs.

% processors, for some tasks, might be executed asynchronously. CPUs and GPUs will begin task execution at the same time, and CPU and GPU micro-batches will just follow the original implementations until they all finish, then the results of all micro-batches could be passed to the downstream of a GL pipeline.

\subsection{Scheduling policy}

% 4 - 5 sentences to motivate
% 1. Motivate the need for training throughput (In SGD, the task must be completed in order, so it is equivalent to minimise task completion time given a batch of input data.....), instead of simplying keeping all devices busy
% 2. Low overhead (policy must be decentralised)

% .....

% \subsection{Scheduling policy design}

% \begin{itemize}
%     \item task finishing time
%     \item async execution
%     \item task interference
% \end{itemize}

The \sys scheduler automatically optimises the size and assignment of the micro-batches from a GL task. To achieve this, it relies on several task performance metrics, which are computed at runtime:

%\sys's parallelism policy models the characteristics of the given workload and improves itself by profiling key metrics, then it will reach the optimal intra-batch parallelism performance. Its workload-aware approach ensures that processor utilisation is higher than a static parallelism scheme. \sys's policy design contains major workload-specific factors in our modelling procedures, which means if the workload has been changed, our policy will still lead the parallelism decision to the optimal one, while a static policy might experience significant performance issues.

\mypar{Task completion time}
% In \sys, we divide the GL pipeline into three major types of computation tasks: (i)~sampling, (ii)~feature aggregation, (iii)~training. The last task is exclusively executed on GPUs, while the other two tasks utilise both CPUs and GPUs. The objective of our parallelism policy is to maximise the end-to-end training time of each task, which is equal to minimising the finishing time for each task.
Task implementations often come from external libraries, and \sys must have metrics to estimate task completion times. Estimating task completion times in GL, however, is challenging. GL tasks exhibit highly diverse resource requirements: graph sampling can be compute-intensive or communication-intensive, depending on hyper-parameters; feature aggregation is often communication-intensive and memory-intensive. Even for the same type of task, completion times may vary. For example, graph sampling for 1-layer neighbours exhibits stable performance; wheres 3-layer neighbours can lead to large differences in sampled graph nodes, thus changing task completion times. To handle this, \sys use the following metric to estimate task completion time:

%because GL tasks might have different computation characteristics on CPUs or GPUs, and theoretical computation throughputs of CPUs and GPUs could not predict the computation time accurately. For example, the graph is sparse and irregular, so sampling could not be fully parallelised on GPUs, but CPUs can parallelise sampling by using multiple cores to generate samples independently. Since we split a batch into micro-batches and dispatch them to CPUs and GPUs, so the task finishing time depends on the processor which finishes its micro-batch in the last place.

\begin{equation}\label{objective}
    % T = \min_{proc \in P}{\mathtt{TASKTIME}(proc, A)}
    \mathcal T_{\mathtt{estimate}} = \min\{\mathcal T_{\mathtt{task}}(pu, A) \mid pu \in P\}
\end{equation}

\noindent
where different types of devices (\ie CPU and GPU) are in the set~$P$ and given a task assignment~$A$. Therefore, \sys can analyse the workload and model the factors in $\mathcal T_{\mathtt{task}}(pu, A)$. In fact, $A$ are the micro-batch sizes for CPU and GPU, so it can be represented as $A_{pu}$ for processor~$pu$. For example, when \sys decides the task assignment of one CPU and two GPUs, $(c, g0, g1)$, given the batch size equal to $1024$, $A$ could be $A_{c}=512, A_{g0}=256, A_{g1}=256$, indicating that the micro-batch sizes are $512$, $256$, $256$ for CPU, GPU~0 and GPU~1, respectively.

%Next we will discuss those factors and how \sys takes them into consideration when designing the policy.

\myparr{Micro-batch size} is another factor that can affect task completion time. In general, the completion time for a GL task is linear with the micro-batch size: similar to other deep learning workloads, the input data dimension can be parallelised efficiently in GL. This property also holds for heterogeneous processors, so we can construct a linear model for CPUs and GPUs for our base completion time:

\begin{equation}\label{base}
    % \mathtt{BASETIME}_{proc} = base_{proc} * A_{proc}
    \mathcal T_{\mathtt{base}}(pu) = base_{pu} * A_{pu}
\end{equation}

In the warm-up phase of a GL job, \sys disables hybrid execution, so that only one type of processor is used. It then obtains an estimate of $\mathit{base}_{pu}$ by averaging the computation time for an interval and inducing this parameter.

\mypar{Asynchronous execution} A unique challenge in estimating task completion time in GL is that of using many devices: both CPU and GPU are used in the asynchronous execution mode, \ie when collective communication  overlaps with training. An accurate task estimation metric must therefore consider the asynchronous nature of many GL tasks.
%\sys assumes that during the execution of a batch, a task might be executed asynchronously.
We observe that GL systems often maintain additional resources, \eg background threads and network communicators, to achieve asynchronous execution. We thus include a coefficient to the ideal background execution interval for an asynchronous GL task:

\begin{equation}\label{async}
    % \mathtt{ASYNCTIME}_{proc} = async\_time^{-\mathit{eff}}
    \mathcal T_{\mathtt{async}}(pu) = async\_time^{-\mathit{eff}}
\end{equation}

\noindent
where $async\_time$ represents the maximum duration for overlapping tasks. It can be obtained by profiling the duration of all other tasks because it is only possible to run a task asynchronously during that time. Due to asynchronous execution overheads, we add $\mathit{eff}$ to \E\ref{async} to capture the behaviour of asynchronous tasks.

% Since this equation does not involve the assignment $A$, \sys could monitor and improve the parameter estimation during training.

\mypar{Data locality} GL tasks often perform intensive data accesses. As a result, data locality becomes important when deciding on task completion time. For example, CPU and GPU sampling tasks may simultaneously access the graph, which is stored in CPU memory, thus affecting each other. Network bandwidth is also shared because all tasks may perform remote requests (\eg sampling a remote subgraph, fetching remote features or performing an all-reduce of gradients). \sys models this behaviour by:

\begin{equation}\label{locality}
    % \mathtt{REMOTETIME} = \sum_{proc \in P}{remote_{proc} * A_{proc}}
    \mathcal T_{\mathtt{remote}} = \sum_{pu \in P}{remote_{pu} * A_{pu}}
\end{equation}

\noindent
where $\mathcal T_{\mathtt{remote}}$ is the global overhead, determined by the task assignment for all processors. When two tasks share the same data transfer path, they alternate in transferring data through the path, and thus roughly finish their data transfer at the same time, albeit with higher latency. \sys considers all processor assignment decisions---the corresponding parameters in the equation can be approximated by profiling the latency increase when launching hybrid tasks on multiple processors.

\begin{equation}\label{total}
    % \mathtt{TASKTIME} = \mathtt{BASETIME} - \mathtt{ASYNCTIME} + \mathtt{REMOTETIME}
    \mathcal T_{\mathtt{task}} = \mathcal T_{\mathtt{base}} - \mathcal T_{\mathtt{async}} + \mathcal T_{\mathtt{remote}}
\end{equation}

\mypar{Task scheduling decisions} Finally, $\mathcal T_{\mathtt{task}}$ can be inferred from \E\ref{total}. Since \sys's task scheduling goal, as described in \E\ref{objective}, is to minimise the task completion time, \sys obtains the optimal micro-batch size assignment, which has the lowest time cost, using a gradient descent method.

\mypar{Scheduling example} The input to \sys's scheduler is the type of a task. If a sampling task (with implementations in~\myc{2}) is to be scheduled on one CPU and two GPUs~(\F\ref{fig:task}), \sys first extracts the policy parameters corresponding to this task (decided by the metrics monitored by sampling execution in~\myc{4}). It then uses the equations above to compute an estimate of task completion time for both CPU and GPU. After that,  \sys adjusts the CPU/GPU micro-batch sizes, \ie the number of input samples for each processor, so that the task finishes quickest.

\subsection{Scheduler implementation}

% The \sys schedulers can collect task performance metrics, and thus can operate based on local workload information, thus preventing the need of using a central scheduler.
% However, a key question here is: how does the decentralised \sys scheduler ensure
% that the cluster-wide training throughput can be benefited based on scheduling decisions made locally?

\mypar{Decentralised architecture} In \sys, each server has its own local scheduler with its own task metrics. The local scheduler makes scheduling decisions based on local information. \sys thus does not rely on a central node to coordinate distributed scheduling decisions. This scheduler design is even more effective than a global scheduler because, in a heterogeneous cluster, each server may be configured differently, which makes a singke global scheduling decision sub-optimal for all servers.

\mypar{Low performance overhead} The granularities of GL tasks are coarse (tens of milliseconds), and \sys does not update the metrics frequently. This means that the scheduling time is amortised throughout a long training period. The scheduling overhead is further reduced by early stopping of the scheduling algorithm if the micro-batch assignment becomes stable.

% Micro-batch dispatching is a light-weight operation, but as the number of servers increases, the cost could be non-negligible if there is only a central coordinator. \sys decentralises the policy execution by running distributed dispatchers on servers, and the profilers are also distributed accordingly. There are one dispatcher and one profiler on each server for intra-server dispatching, and inter-server dispatching is only decided at the beginning, which will greatly reduce policy execution overheads compared with having a global dispatcher. All dispatchers will run in parallel with their own local policy parameters and the profiler will sample necessary metrics and send them to local dispatcher periodically, so no global synchronisation is required. The profilers only collect intra-server metrics, and the profiled metrics will not be synchronised globally. In the end, the policy parameters from different servers could diverge, but in practice this will not affect the effectiveness of our policy.
%
% Another advantage of decentralised policy execution is the effectiveness when the servers are highly heterogeneous in the cluster (\eg imbalanced network topology or servers with different processor configurations). In this case, it is challenging to have a global policy that is adaptive to heterogeneous servers, but \sys's decentralised policy execution will make each server's policy commodate its own conditions.

% End


==> tables/experiment.tex <==
\begin{tabular}{|l|l|l|l|l|}
    \hline
    Experiment                  & Criteria                  & Model         & Datasets      & Test-bed  \\
    \hline
    scalability (single server) & end-to-end epoch time     & GraphSage    &  paper100M,ogbn-products,mag240M    & (i)\\
    \hline
    scalability (multiple servers) & end-to-end epoch time     & GraphSage,GAT &  paper100M,mag240M & (i),(ii) \\
    \hline
    data access                   &      hit ratio          &         N/A     &     paper100M &    N/A    \\
    \hline
    task scheduler                 &     throughput         &   GraphSage     &      N/A      &  N/A \\
    \hline
    unified tensor                 &     throughput         &   N/A     &      paper100M,mag240M     &  N/A \\
    \hline
\end{tabular}

==> tables/out-of-core.tex <==
% Out of core table

\begin{tabular}{crr}\toprule
\textbf{\#GPUs} & \textbf{DGL} & \textbf{\sys} \\\midrule
1 & 14,500\unit{s} &	416\unit{s} \\
2 & 13,200\unit{s} &	193\unit{s} \\
3 & 11,990\unit{s} &	41\unit{s} \\
4 & 11,210\unit{s} &	10\unit{s} \\\bottomrule
\end{tabular}

